Bayesian Poisson Mortality Projections with Incomplete Data

The missing data problem pervasively exists in statistical applications. Even as simple as the count data in mortality projections, it may not be available for certain age-and-year groups due to the budget limitations or difficulties in tracing research units, resulting in the follow-up estimation and prediction inaccuracies. To circumvent this data-driven challenge, we extend the Poisson log-normal Lee-Carter model to accommodate a more flexible time structure, and develop the new sampling algorithm that improves the MCMC convergence when dealing with incomplete mortality data. Via the overdispersion term and Gibbs sampler, the extended model can be re-written as the dynamic linear model so that both Kalman and sequential Kalman filters can be incorporated into the sampling scheme. Additionally, our meticulous prior settings can avoid the re-scaling step in each MCMC iteration, and allow model selection simultaneously conducted with estimation and prediction. The proposed method is applied to the mortality data of Chinese males during the period 1995-2016 to yield mortality rate forecasts for 2017-2039. The results are comparable to those based on the imputed data set, suggesting that our approach could handle incomplete data well.

==> Data.tex <==
\section{Estimation and Prediction Results} 

\hspace{12pt} The appropriate starting values play an important role in the rate of convergence. We follow the procedures of getting them: 
\begin{enumerate}
\item Use linearly interpolating to impute all missing $D_{x,t}$ and $E_{x,t}$.
\item Obtain crude estimates of the parameters in the LC model by the SVD method.

\item Utilize the multiple imputation method proposed by~\citet{Czado} to impute all missing data again. 
\item Use the estimates from step 2 as initial values, apply the methodology to update estimates in the proposed model for the complete data made by the last step. 
\end{enumerate}

By implementing all above steps, we obtain initial values of all parameters in our proposed model for the incomplete data. We set $a_{\sigma_{\alpha}^2} = b_{\sigma_{\alpha}^2} = a_{\sigma_{\beta}^2} = b_{\sigma_{\beta}^2} = 0.01$ as age-related hyperparameters, and consider $a_{\zeta}$ = $b_{\zeta} = 0.1$ for the random scalar $\zeta$. Note that we tried different constants to replace 0.01 and 0.1  in~(\ref{eqn:3.11}) and~(\ref{eqn:3.12}), we found that a substantial change does not appear in the posterior inferences.

We apply a Gibbs sampler algorithm to obtain draws in~\autoref{fig:1} from the full conditional posterior distribution for $\theta_2$. 

 

\captionsetup[figure]{labelfont={bf},labelformat={default},labelsep=period,name={Fig.}}
\begin{figure}[H]
    \centering
    \includegraphics[height=10cm,width=15cm]{7-7.pdf}
    \caption{\label{fig:1}Plot of the chain for $\theta_2$ }
\end{figure}


From the last 500 draws, we estimate a posterior mean 0.00409, $95\%$ Highest Density Interval (HDI) $(-0.01,0.03)$ and $95\%$ Equal-tailed Interval (ETI) $(-0.01,0.04)$. Due to the difficulties in obtaining the marginal likelihood in the proposed model, it is complicated to calculate the Bayes factor. So we use $95\%$ credible intervals to conclude that $\theta_2$ is not significantly different from zero, meaning for this incomplete data set we fail to reject $H_0$ and the random walk model with drift is preferable. 

Before applying the methodology for the incomplete data to estimate the parameters in the proposed model, we iterate 2000 times for $\sigma_{x,t}^2$.~\autoref{fig:2} shows the selected $\sigma_{x,t}^2$ and corresponding acceptance rates for the years 2000 and 2010, in which we have the complete data set for all age groups. We observe that proposal variances have a similar pattern for different years.  
\clearpage
\begin{figure}[H]
    \centering
    \includegraphics[height=15cm,width=15cm]{1.pdf}
    \caption{\label{fig:2}Plots of proposal variances and the acceptance rates for year 2000 and 2010}
\end{figure}



~\autoref{fig:3} gives separate chains of parameters for selected age 50 and year 2000. These plots show that the chains converge well. The initial values improve the convergence successfully. Clearly, after the first 50 runs all chains are asymptotic. 

\begin{figure}[H]
    \centering
    \includegraphics[height=23cm,width=15cm]{2.pdf}
    \caption{Plots of separate chains for a subset of parameters in the Proposed model}
    \label{fig:3}
\end{figure}


In the presence of missing data,the following three figures depict estimates of $\alpha_x$'s, $\beta_x$'s and $\kappa_t$'s in the proposed model. From~\autoref{fig:4} and~\autoref{fig:5}, we see that the patterns of the estimated $\alpha_x$ and the estimated $\beta_x$ are similar. On the contrary,~\autoref{fig:6} shows that there are significant differences between the pattern of $\kappa_t$ and the pattern of $\beta_x$, as well as the pattern of $\kappa_t$ and the pattern of $\alpha_x$. These two features are the result of constrains~(\ref{eqn:3.2}). From the linear transformation~(\ref{eqn:2}), we have $d=1$ and $c= - \sum_x \alpha_x$ to keep invariant mortality projections. So, the estimated $\alpha_x$'s have special relationship with the estimated $\beta_x$'s. 


\begin{figure}[H]
    \centering
    \includegraphics[height=4.5cm,width=15cm]{3-3.pdf}
    \caption{Estimations of $\mathbold{\beta}$}
    \label{fig:4}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[height=4.5cm,width=15cm]{4-4.pdf}
    \caption{Estimations of $\mathbold{\alpha}$}
    \label{fig:5}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[height=4.5cm,width=15cm]{5-5.pdf}
    \caption{Estimations of $\mathbold{\kappa}$}
    \label{fig:6}
\end{figure}


We choose four different age groups to present a graph of the observed log mortality rates for year 1995-2016 along with the point estimate of the forecast and $95\%$ prediction intervals for year 2017-2039 by sampling iteratively.~\autoref{fig:7} shows that when age is higher, the predicted log mortality rates decrease slower, and the differences between upper bound and lower bound of the $95\%$ confidence intervals increase slower.







\begin{figure}[H]
    \centering
    \includegraphics[height=14cm,width=15cm]{6-6.pdf}
    \caption{Observed (black points) and predicted log mortality rates with $95\%$ prediction intervals(dash line) for Chinese males }
    \label{fig:7}
\end{figure}

==> Date2.tex <==
\section{Data} \label{Data Analysis}

\hspace{12pt} We follow ~\citet{Claudia} to get estimators of $\mathbold{\kappa, \beta, \alpha}, \kappa_0, \theta and \sigma_{\omega}^2$ by using Kalmer filter and Gibbs sampler in standard LC model (1)&(4) with constrain (2), then adjust their estimators by (5) and use adjusted estimators as the starting point of MCMC in PLC model (3)&(4) with constrain (5). 

